Convex Hull Formulations for Mixed-Integer Multilinear Functions

In this paper, we present convex hull formulations for a mixed-integer, multilinear term/function (MIMF) that features products of multiple continuous and binary variables. We develop two equivalent convex relaxations of an MIMF and study their polyhedral properties in their corresponding higher-dimensional spaces. We numerically observe that the proposed formulations consistently perform better than state-of-the-art relaxation approaches.

==> Sections/Conclusions.tex <==
\section{Conclusions}

MIMFs are a class of non-convex functions that arise in a wide variety of optimization problems. In this paper, we consider MIMFs and develop new convex relaxations based on the convex hull of the disjunctive union of these two sets of variables in an extended space. We also empirically showed the superiority of the convex hull formulation over state-of-the-art approaches. While this paper has made strides in tightening relaxations of MIMFs, there remain a number of important future directions including the characterization of the convex hull of MIMFs in the space of it's original variables. 

